TCT: Convexifying Federated Learning using Bootstrapped Neural Tangent Kernels

State-of-the-art federated learning methods can perform far worse than their centralized counterparts when clients have dissimilar data distributions. For neural networks, even when centralized SGD easily finds a solution that is simultaneously performant for all clients, current federated optimization methods fail to converge to a comparable solution. We show that this performance disparity can largely be attributed to optimization challenges presented by nonconvexity. Specifically, we find that the early layers of the network do learn useful features, but the final layers fail to make use of them. That is, federated optimization applied to this non-convex problem distorts the learning of the final layers. Leveraging this observation, we propose a Train-Convexify-Train (TCT) procedure to sidestep this issue: first, learn features using off-the-shelf methods (e.g., FedAvg); then, optimize a convexified problem obtained from the network's empirical neural tangent kernel approximation. Our technique yields accuracy improvements of up to +36% on FMNIST and +37% on CIFAR10 when clients have dissimilar data.

==> editor.tex <==
\usepackage[normalem]{ulem}
\usepackage{xcolor}


\newcommand{\add}[1]{{\color{red!70!black} #1}}
\newcommand{\del}[1]{{\color{red!50} \sout{#1}}}
\newcommand{\rep}[2]{{\color{blue!50} \sout{#1}}{\color{blue!70!black} #2}}
\newcommand{\cmt}[2]{{\color{red!15!blue!65} #1}\footnote{{\color{red!60!black} $\leftarrow$ #2}}}
\newcommand{\gram}[1]{{\color{red!70!gray} {\bfseries #1}}}
\newcommand{\hlt}[1]{\gram{#1}}

\newcommand{\scrcmd}{\textsuperscript}
\newcommand{\scr}[1]{\scrcmd{#1}}
\newcommand{\myst}{{\hypersetup{hidelinks}\bf \color{purple} \hyperref[exp:myst]{\scr{mysterious}}}}
\newcommand{\cit}{{\hypersetup{hidelinks}\bf \color{green!50!black} \hyperref[exp:cit]{\scr{cite}}}}
\newcommand{\wdy}{{\hypersetup{hidelinks}\bf \color{orange} \hyperref[exp:wdy]{\scr{wordy}}}}
\newcommand{\unimp}{{\hypersetup{hidelinks}\bf \color{blue!70} \hyperref[exp:unimp]{\scr{unimportant}}}}
\newcommand{\awk}{{\hypersetup{hidelinks}\bf \color{red} \hyperref[exp:awk]{\scr{awkward}}}}

\newcommand{\ExplanationPage}{
\newpage
\onecolumn

\section*{Explanation of editor markings}
\renewcommand{\scrcmd}{}
\hypersetup{hidelinks}
\begin{itemize}
\item \label{exp:myst} \myst: This will probably come across as mysterious to readers who don't already have the context to know what you're talking about.
\item \label{exp:cit} \cit: You should try to cite something here (e.g. to give an example of, or justification for, what you just talked about).
\item \label{exp:wdy} \wdy: This is stated in more words than is necessary and can probably be shortened.
\item \label{exp:unimp} \unimp: This is not that important relative to the length/prominence it's currently given.
\item \label{exp:awk} \awk: Awkward grammar (overly complex and/or not clear what a given subclause/modifier corresponds to).
\end{itemize}
}


==> understanding.tex <==
\section{Understanding}\label{sec:understanding}
TODOs:
\begin{enumerate}
    \item Two layer toy model?
    \item Visualize weight magnitude of learned linear models on eNTK?
\end{enumerate}



